Towards Hyperparameter-free Policy Selection for Offline Reinforcement Learning

How to select between policies and value functions produced by different training algorithms in offline reinforcement learning (RL) -- which is crucial for hyperpa-rameter tuning -- is an important open question. Existing approaches based on off-policy evaluation (OPE) often require additional function approximation and hence hyperparameters, creating a chicken-and-egg situation. In this paper, we design hyperparameter-free algorithms for policy selection based on BVFT [XJ21], a recent theoretical advance in value-function selection, and demonstrate their effectiveness in discrete-action benchmarks such as Atari. To address performance degradation due to poor critics in continuous-action domains, we further combine BVFT with OPE to get the best of both worlds, and obtain a hyperparameter-tuning method for Q-function based OPE with theoretical guarantees as a side product.

==> misc.tex <==


We also consider different variants of the BVFT algorithm to compare their performance:
\begin{itemize}[leftmargin=0.5cm]
    \item BVFT best: We select an array of candidate resolutions and run the single resolution version of BVFT as described in Algorithm \ref{bvft_algo_1} to obtain an ordinal ranking for each resolution. We then use the ground truth ranking to select the resolution which has the best-ranking performance as a skyline for the performance of BVFT using a single fixed resolution for all function pairs.
    \item BVFT auto: This is the variant of the original BVFT described in Algorithm \ref{bvft_algo_2} where the resolution for each policy is automatically selected as the minimizer of the loss.
    \item Hybrid: A linear combination of statistics calculated by BVFT best and Avg$Q(s,a)$ where the combination parameter is optimized through line search to form a skyline. Here we want to see the upper bound of how well Avg$Q(s,a)$ and BVFT's combination would perform.
\end{itemize}


\section{Misc}
\subsection{Approach}
Xie and Jiang \cite{xie2020batch} recently proposed Batch Value Function Approximation (BVFT) for batch (offline) reinforcement learning. With the assumption on only exploratory data and realizable arbitrary function class, BVFT is the first algorithm that theoretically achieves polynomial-sized sample efficiency on learning the $Q^*$ function from batch data. BVFT works by applying a tournament procedure to the set of functions in the class, reducing the learning problem to that of identifying $Q^*$ from a pair of candidate functions. Although the pairwise comparison in the tournament procedure poses a significant computational burden and may be intractable for rich function classes such as deep neural networks, BVFT can be used efficiently for the task of policy selection in offline RL. In this thesis, we investigate the performance of BVFT when used for the task of offline policy selection. In addition, we propose several modifications to BVFT to better fit empirical application and adaptation to various RL environments.

\subsection{Batch Value Function Tournament (BVFT)}
We first introduce the originally BVFT algorithm proposed by Xie et al. \cite{xie2020batch}. The idea of BVFT was inspired by previous research in state-abstraction: with the function class $\mathcal{F}$ being a piecewise constant and realizable function class, batch learning is consistent using Fitted Q-iteration with exploratory data. In order to fit the piecewise constant property on commonly used function class such as linear classes or neural networks, Xie. et al proposed to augment $\mathcal{F}$, which is not piecewise constant, to its smallest superset that is piecewise constant, while still being realizable. As described in Algorithm \ref{bvft_algo_1}, BVFT first discretizes the output of each Q-value function $f \in \mathcal{F}$ up to a small discretization error $\epsilon_{dct}$. Then for each pair of value functions in $\mathcal{F}$, BVFT partitions the state-action space $\mathcal{S} \times \mathcal{A}$ into $\phi$ by grouping state-action pairs together only when the output of both functions are constant across them. The reason behind the pairwise comparison is due to the number of groups in the partition can be as large as $(V_{\text{max}}/\epsilon_{dct})^{|\mathcal{F}|}$. Without reducing $\mathcal{F}$ to 2, the statistical complexity is doubly exponential in poly log $|\mathcal{F}|$. 

After constructing a piecewise constant class $\mathcal{G}_{\phi} \subset (\mathcal{S} \times \mathcal{A} \rightarrow [0, V_{\text{max}}])$, BVFT then calculates $||f_0 - \hat{\mathcal{T}}^{\mu}_{\phi}f_0||_{2,D}$ as a surrogate for $|| f_0 - Q^*||$ where $\hat{\mathcal{T}}^{\mu}_{\phi}$ is the projected Bellman update operator associate with $\mathcal{G}_{\phi}$. The pairwise comparison allows efficient elimination of Q-functions that are farther away from $Q^*$, allowing the ranking of candidate Q-value functions with respect to their distance from $Q^*$. For detailed explanation and proof behind BVFT, please refer to the original paper \cite{xie2020batch}.\\

\begin{algorithm}[H]
\SetAlgoLined
\KwIn{Dataset $D$, value-functions set $\mathcal{F}$, discretization parameter $\epsilon_{dct} \in (0, V_{max})$}
\For{$f \in \mathcal{F}$}{
$\Bar{f} \leftarrow$ discretize the output of $f$ with resolution $\epsilon_{dct}$.
}
 \For{$f \in \mathcal{F}$}{
 \For{$f' \in \mathcal{F}$}{
  Define $\phi$ s.t. $\phi (s', a')$ iff $\Bar{f}(s, a) = \Bar{f}(s', a')$ and $\Bar{f'}(s, a) = \Bar{f'}(s', a')$\;
  Let $\mathcal{G}_{\phi} \subset (\mathcal{S} \times \mathcal{A} \rightarrow [0, V_{\text{max}}])$ be the piecewise constant function class induced by $\phi$, a partition of $\mathcal{S} \times \mathcal{A}$\;
  $\hat{\mathcal{T}}^{\mu}_{\phi}f := \text{argmin}_{g\in \mathcal{G}_{\phi}} \frac{1}{|D|} \sum_{(s,a,r,s')\in D} [(g(s,a) - r - \gamma V_f (s'))^2]$ \;
  $\mathcal{E}(f$; $f') \leftarrow ||f - \hat{\mathcal{T}}^{\mu}_{\phi}f||_{2,D}$\; 
 }
 $f_l \leftarrow \text{max}_{f' \in \mathcal{F}}\mathcal{E}(f$;$f')$\;
 }
 \KwOut{$\mathcal{O} \leftarrow \text{ArgSort}(\{ f_l, \forall f \in \mathcal{F}\})$} 
 \caption{Batch Value-Function Tournament (BVFT) for Policy Selection}
 \label{bvft_algo_1}
\end{algorithm}

\subsection{Application to Model Selection}
In empirical machine learning it is a common practice to experiment with different algorithms, as well as grid searching function approximators architectures, hyper-parameters to see which combination produce the best performance. In supervised learning, this process is usually done by running all models on the validation while in online RL such model selection can be done by running all models in the environment and selects the one with the highest value. However, in the offline RL setting, this becomes a very challenging and still open problem. BVFT's offers a direct approach to this problem: by running BVFT on a set of candidate functions  $\mathcal{F}$, the tournament procedure allows the selection of the policy that is the closest to $Q^*$ as well as a ranking based on the statistics BVFT calculates, which is a surrogate for $|| f - Q^*||$.

\paragraph{Selection of discretization resolution}
When applying BVFT empirically to offline policy selection, the choice of the discretization resolution $\epsilon_{dct}$ becomes tricky: if the resolution is too large, the low number of groups in the partition would cause the state abstraction to be very coarse to produce accurate results. On the other hand, if the resolution is too low then the state abstraction would be too fine to produce any meaningful groups. In this case, the statistics we calculate would be equivalent to the one sample-based Bellman-residual which was shown to break down in environments with more stochastic transition dynamics \cite{deterministic_br}. To address this parameter choice, we propose BVFT with automated resolution selection detailed in Algorithm \ref{bvft_algo_2}. In this approach, instead of providing only one discretization resolution, the algorithm takes a set of potential discretization resolutions. In practice, a simple choice of this set can be a series of values in exponential relationship, i.e. $\{2^i\}_{i = c}^{c+k}$ where $c$ is the starting exponent and k is the number of resolutions to consider. After running the pairwise tournament procedure over all the resolutions to calculate the statistics, we then take the minimum with regularization on the resolution to be the aggregated statistics of the function. At the end, functions are simply sorted based on their aggregated statistics to deliver the ranking. The advantage of using this approach is obvious: replying on a single resolution would require a careful choice of the parameter but in the offline setting there is simply no way of verifying the performance based on this choice. With automated resolution, the resolution is automatically chosen by the minimizer of the statistics of each function. In addition, all pairs of functions no longer have to use the same resolution and the minimizer can optimize the resolution for each pair of functions. We experimented with this version of BVFT in comparison with the previous version of the single fixed resolution, with the result in the next chapter.\\

\paragraph{Adaptation to continuous action space domain}
For domains with continuous action space, policies can not be directly derived from the value function by taking the argmax across all possible actions, as there are an infinite amount of possible actions. Instead, popular learning algorithms \cite{lillicrap2019continuous, mnih2016asynchronous, haarnoja2018soft} often learns 2 functions: The actor function $f_A \rightarrow \mathcal{A}$ either learns a policy that directly outputs an action or a distribution of action and samples from it. The critic function $f_C \rightarrow \mathcal{S} \times \mathcal{A}$ learns the q-value for each state-action pair which measure the utility. The learning algorithm typically optimizes both functions simultaneously during the learning phase. When applying BVFT to models learned using both actor and critic function, a slight modification to the algorithm is necessary: Since taking the maximum of the value function of a state overall actions is infeasible, we instead take the action produced by the actor function $f_A$ and then estimated the value of the next state using $V_f(s') = f_C(s', f_A(s'))$. The intuition behind this is that since the goal of the actor function is to learn or propose the action that would maximize the future utility, then using its action of choice should be equivalent to taking the argmax over actions in value-based RL algorithms. 

\paragraph{In combination with other OPE approach}
We also propose the usage of BVFT in combination with other OPE-based approaches in order to further boost the performance. Although OPE based approaches such as Fitted-Q evaluation \cite{le2019batch} has limitations of often requires more data for regression due to the complexity of its rich function class, while being sensitive to its own choice of hyper-parameters, they also have the advantage of directly estimating policy value instead of using $||f - Q^*||$ as a surrogate. Paine et al. also recently shown that the value estimate in an actor-critic type of algorithm can be significantly overestimated \cite{paine2020hyperparameter} and the value function estimated by Fitted-Q evaluation can significantly reduce such over-estimation. Thus we propose to combine both approaches and feed the value function estimated by the OPE-based approach to BVFT for policy selection in the continuous action domain. Another approach is to use a linear combination of the loss produced by BVFT with value estimates from other metrics to boost the performance of policy selection. We investigate the performance of these proposed methods in our experiments.

\paragraph{Theorem 1}
If the minimum amount of data in each group of state action pairs: $\mu^{\phi}_{min}$ is at least $\frac{1}{C}$, then Theorem 2 in the original paper still holds.


We empirically evaluate BVFT in a number of RL environments \cite{openai} and public datasets \cite{gulcehre2021rl, fu2021d4rl} for the task of offline policy selection in both tabular and function approximation setting. We want to study the performance of BVFT and other Offline Policy Selection algorithms under various conditions with a number of domain characteristics in mind. More specifically, we consider the effect of environment complexity, environment stochasticity, dense vs. sparse reward, algorithm hyper-parameter setting, length of the horizon, size, and diversity of the dataset on the performance of the OPC methods.

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{cs_thesis_latex_template-2020/envs_illustration.png}}
% \caption{our experiment environments ranges from simple discrete grid world like (a) Taxi to complex domains such as (d) Atari 2600 Games where observation space is extremely high dimension pixel space with long horizon, stochastic dynamics and sparse rewards.}
% \label{envs}
% \end{center}
% \vskip -0.2in
% \end{figure}



\subsection{Discussion}
As a Bellman Residual Minimization (BRM) based method, BVFT approaches this problem from a completely different angle compared to most of the OPE-based method. It has the advantage of requiring less data, as well as not relying on picking the correct hyper-parameter for itself and hard optimization problem posed by many popular regression-based OPE approach. However, BVFT posses its own limitations. In this chapter, we will discuss a few caveats when applying the BVFT algorithm as well as potential future directions.

\subsection{Limitation of the Method}
First of all, BVFT is a BRM-based method that evaluates the performance of models by going through $||f - Q^*||$ as a surrogate instead of directly estimating the value function of the evaluation policy. This makes BVFT relying on that the base algorithms to need to approximate $Q^*$ which limits its applicability. For instance, in the continuous action space domain such as MuJoCo, popular learning algorithms often prioritize learning the policy function. Even with actor-critic models, the critic's convergence is often much slower than the policy, resulting in much less accurate value estimation even when the policy has near-optimal performance. In such a case, OPE-based methods such as FQE as a big advantage, and BVFT would need to rely on the more accurate estimation produced by these methods, limiting its application. In addition, in some environments due to various factors such as reward design, termination condition, etc., the correlation between $||f - Q^*||$ and the policy's actual performance might not be strong enough to allow an accurate estimation.

OPE-based method also has its advantage of directly estimating the policy value, which BVFT can not offer. This information can be valuable to several applications where an accurate estimation of the performance is necessary before actually deploying the models. Regression-based OPE method enjoys another advantage of well-developed automated differential packages \cite{NEURIPS2019_9015} which enables high capacity function approximators to efficiently generalize based on large amounts of data. On the other hand, BVFT requires pairwise comparisons between each function in the set, and as the number of models grows, the asymptotic run time would be $\mathcal{O}(n^2)$, although this can be lower down through divide and conquer, the overall computation still grows at a higher rate with respect to the number of policies.

\subsection{Conclusion}
We applied the BVFT algorithm, a polynomial sample complexity batch RL learning algorithm, to the task of offline model selection in reinforcement learning. We proposed several modifications to the original algorithm to better fit the purpose of offline model selection. We experimented BVFT along with a number of popular baselines in a wide variety of RL environments in different settings. From the results, we observe that BVFT has good and reliable overall performance and outperforms baselines by a margin in many of the environments. We address several important factors that can affect the performance of the various methods in the task of model selection. We hope researchers who are interested in this problem can find this work useful for further work in this direction.



\section{Related work}
Offline policy selection has been a long-standing and intensely studied problem in reinforcement learning due to its critical role in offline reinforcement learning. It has a wide spectrum of applications in real-life ranging from recommendation systems \cite{Li_2010, Dud_k_2014, the2015}, to robotics \cite{kalashnikov2018qtopt, irpan2019offpolicy}, and healthcare systems \cite{raghu2018behaviour, nie2020learning, gottesman2020interpretable}. Pioneers of the offline RL algorithms include fitted Q iteration \cite{ernst2005tree, riedmiller2005neural} as well as the least square temporal difference algorithm \cite{bradtke1996linear, lagoudakis2003least}. More recent work on offline RL methods introduces a number of algorithms \cite{agarwal2020optimistic, kumar2019stabilizing, fujimoto2019offpolicy, siegel2020doing} which outperform the previous offline RL models by a large margin. Novel methodologies also seek to tackle the problem of extrapolation error \cite{fujimoto2019off}. In addition, there has been a number of offline RL datasets developed for bench-marking learning and evaluation algorithms \cite{fu2021d4rl, gulcehre2021rl}.

\subsection{Offline Policy Selection}
The offline policy selection problem we study in this thesis is a decision problem that falls into the category of model selection problem in machine learning. The main application of model selection in recent machine learning research is to perform hyper-parameter tuning to improve the performance of the model on various tasks \cite {li2017hyperband, jaderberg2017population}. Bergstra et al. demonstrated that the performance of deep learning models can be improved even with just a random search based on a simple heuristic. Recent work has also shown that many of the sophisticated language models that were claimed to be state-of-the-art can be outperformed by much simpler LSTM models but with properly tuned hyper-parameters \cite{melis2017state}.

Model selection in online RL has been a relatively easy task and can be done accurately using Monte Carlo rollouts. However, such a task in the offline RL setting has been a very challenging but yet under-explored area of research. Farahmand et al. \cite{farahmand2011model} introduced the Bellman-error minimization(BerMin) method for offline model selection including theoretical proof and convergence properties. The term policy selection work also refers to the selection of features and learning methods \cite{foster2019model, pacchiano2020model} as well as state abstraction selection \cite{jiang2015abstraction, jiang2017theory}. Recent work \cite{fu2021d4rl, gulcehre2021rl} introduced new methods to evaluate how concrete and RL algorithms are when generalizing to a specific domain without hyper-parameter fine-tuning. Such protocols provided standardized experiment environments to evaluate offline RL algorithms and perform domain adaptation. 

Recently Yang et al. \cite{yang2020offline} formally defined the task of offline policy selection and proposed BayeDice to estimate belief distribution for this task. Several earlier works also focused on a similar setting where the goal is to select out the function approximation that is closest to the optimal Q-value function from a set of candidate functions \cite{fard2010pac, xie2020batch}. The metric to measure the closeness between candidate function and the optimal Q-value function is typical $L_{\infty}$ norm since the assumption is that this metric is correlated with the model's performance. Irpan et al. \cite{irpan2019offpolicy} proposed off-policy classification which directly performs positive-unlabeled (PU) classification based on binary rewards to select policies and experimented in the control domain of RL. Recently Paine et al. \cite{paine2020hyperparameter}also introduced a similar setting of hyper-parameter selection in RL and performed a thorough benchmark on various state-of-the-art offline learning algorithms and policy evaluation algorithm. Compare to these works, our work proposed a novel method to select near-optimal policy using offline data.

\subsection{Off-policy evaluation}
Off-policy evaluation (OPE) has been studied intensely and is closely related to the problem we study in this thesis. OPE was proposed at first to solve the offline policy selection problem \cite{precup2000eligibility} but later the focus has shifted to a similar task of estimate the cumulative rewards of a policy using offline data. In this task, the main goal is either to compute a point estimation of the ground truth expected value of the policy in the online environment \cite{dudik2011doubly, charles2013counterfactual, jiang2016doubly, thomas2016dataefficient, nachum2019dualdice, kallus2020double, uehara2020minimax}, or provide a confidence interval or a lower bound on the policy value \cite{thomas2015high, hanna2018bootstrapping, kuzborskij2020confident, feng2020accountable, jiang2020minimax}.

OPE methods have been categorized into 3 groups: importance sampling, direct methods, and doubly robust methods. The key idea of importance sampling is to re-weight the rewards from the offline data based on the probability ratio of action between the behavior policy and the policy to be evaluated, i.e, the likelihood of receiving each reward under different policies. The advantage of importance sampling is that it offers an unbiased and consistent estimation of the policy value. However, the cumulative product of importance weight throughout each trajectory poses exponential variance with respect to the length of the horizon, causing the method to be unstable in long-horizon tasks. Recently, marginalized importance sampling  \cite{liu2018breaking, xie2020optimal} has been proposed to tackle the exponential variance by estimating the state marginal distribution for the target policy at every step.

Direct methods differ from importance sampling methods by focusing on directly estimating the value function or Q-value function of the policy using regression-based techniques. This category can be further partitioned into model-based approaches and model-free approaches. The former approach directly estimates the transition function, reward function, and termination conditions from offline data which then used to perform Monte-Carlo policy evaluation to estimate the policy value. Model-free methods instead directly estimate the Q-value function of the policy. Direct methods have relatively lower variance compare to importance sampling-based methods but are subject to model miss-specification problems and the estimate is biased. Doubly robust methods tend to combine techniques from both importance sampling and direct methods. Munos et al. \cite{munos2016safe} proposed Retrace that leverages multi-step product of importance weights for off-policy Q-correction. Thomas et al. \cite{thomas2016dataefficient} recently introduced MAGIC which switches between importance weights and direct methods. Voloshin et al. \cite{voloshin2019empirical} performed benchmarks of various state of the art OPE methods in a number of environments and the results indicate that direct methods tend to perform the best in many cases.


==> relatedworks.tex <==



